Testing Research Software: A Survey

Background: Research software plays an important role in solving real-life problems, empowering scientific innovations, and handling emergency situations. Therefore, the correctness and trustworthiness of research software are of absolute importance. Software testing is an important activity for identifying problematic code and helping to produce high-quality software. However, testing of research software is difficult due to the complexity of the underlying science, relatively unknown results from scientific algorithms, and the culture of the research software community. Aims: The goal of this paper is to better understand current testing practices, identify challenges, and provide recommendations on how to improve the testing process for research software development. Method: We surveyed members of the research software developer community to collect information regarding their knowledge about and use of software testing in their projects. Results: We analysed 120 responses and identified that even though research software developers report they have an average level of knowledge about software testing, they still find it difficult due to the numerous challenges involved. However, there are a number of ways, such as proper training, that can improve the testing process for research software. Conclusions: Testing can be challenging for any type of software. This difficulty is especially present in the development of research software, where software engineering activities are typically given less attention. To produce trustworthy results from research software, there is a need for a culture change so that testing is valued and teams devote appropriate effort to writing and executing tests.

==> novelty_statement.tex <==
\textbf{Novelty Statement}
This paper reports on new results that have not appeared in previous publications.
The contents of this paper are novel.

==> table_testing.tex <==
\begin{tabular}{p{\linewidth}}
\hline
Unit testing (87),
Integration testing	(43),
Regression testing (39),
Continuous integration (33),
Test-driven development (18),
Code coverage	(16),
System testing	(14),
Fuzz testing	(12),
Acceptance testing	(9),
validation testing	(9),
Performance testing	(6),
mock testing	(6),
Memory testing	(6),
Static analysis	(6),
Functional testing	(6),
Mutation testing	(5),
black box testing	(4),
Assertions testing	(3),
Documentation checking	(3),
Dynamic testing	(3),
CTest	(3),
Formal Methods	(2),
End-to-end testing	(2),
Random input testing	(2),
White box testing	(2),
Method of manufacture solution	(2),
Property-based testing	(2),
Scientific testing	(2),
Manual testing	(2),
User testing	(2),
Smoke test	(2),
Approval testing	(2),
Visual studio	(2),
Code reviews	(2),
Usability testing	(1),
Install testing	(1),
Reliability testing	(1),
Compatibility Testing	(1),
Load testing	(1),
Agile	(1),
Stress test	(1),
doctests	(1),
test suites	(1),
Golden master testing	(1),
Physics testing	(1),
Benchmarking	(1),
Automatic test-case generation	(1),
Use case test	(1),
Concolic testing	(1),
equivalence class	(1),
n-version	(1),
Beta testing	(1),
Alpha testing	(1),
A/B testing	(1),
Security testing	(1),
Behavioral testing	(1),
Linting	(1),
Code style checking	(1),
Dependencies testing	(1),
Resolution testing	(1),
Comparison with analytical solutions	(1),
Built environment testing	(1),
Contracts	(1),
Jenkins automated testing	(1),
License compliance	(1),
Exploratory tests	(1),
Correctness tests	(1),
run-time instrumentation and logging	(1),
Profiling	(1),
Deployment testing	(1),
Nightly	(1),
Release	(1),
DBC	(1),
reference runs on test datasets	(1),
Checklist testing	(1),
gtest	(1),
jUnit	(1),
Squish	(1),
Caliper	(1),
Bamboo	(1),
GitLab	(1),
Periodic testing	(1),
Pre-commit	(1),
Design by contract	(1),
Statistical testing	(1),
Builtd testing	(1),
Bit-for-bit	(1),
Engineering tests	(1),
Method of exact solutions	(1),
Answer testing	(1),
Behavior-Driven Developent	(1),
Coding standards	(1),
Accuracy testing	(1),
Monitoring production apps	(1),
Asan	(1),
Tsan	(1),
Msan	(1),
Penetration testing	(1),
Checksum	(1)
\hline
\end{tabular}
